ProbeSim: Scalable Single-Source and Top-k SimRank Computations on Dynamic Graphs

Single-source and top-$k$ SimRank queries are two important types of similarity search in graphs with numerous applications in web mining, social network analysis, spam detection, etc. A plethora of techniques have been proposed for these two types of queries, but very few can efficiently support similarity search over large dynamic graphs, due to either significant preprocessing time or large space overheads. This paper presents ProbeSim, an index-free algorithm for single-source and top-$k$ SimRank queries that provides a non-trivial theoretical guarantee in the absolute error of query results. ProbeSim estimates SimRank similarities without precomputing any indexing structures, and thus can naturally support real-time SimRank queries on dynamic graphs. Besides the theoretical guarantee, ProbeSim also offers satisfying practical efficiency and effectiveness due to several non-trivial optimizations. We conduct extensive experiments on a number of benchmark datasets, which demonstrate that our solutions significantly outperform the existing methods in terms of efficiency and effectiveness. Notably, our experiments include the first empirical study that evaluates the effectiveness of SimRank algorithms on graphs with billion edges, using the idea of pooling.

==> existingworks.tex <==
\section{Existing Works}
This section revisits existing methods which can be used for the single source top-$k$ SimRank query directly or undirectly. Generally these works can be categorized as follows, according to their relevance to our problem: \\
(I) Directly computes single source top-$k$ SimRank; \\
(II) Efficiently compute single pair or single source SimRank. Once we get $s(u,v)$ for all $u \neq v$, only a sorting procedure is needed to retrieve the $k$ largest scores, using $O(n)$ space and extra $O(n\mathrm{log}n)$ time; \\
(III) Firstly compute all-pair SimRank and then get the $k$ largest values with respect to the given vertex $v$. Obviously this kind of methods is more time and space expensive than previous two types.
\subsection{Single Source Top-$k$ SimRank}
The only known method of type I is TopSim \cite{LeeLY12}, which exactly solve the single source top-$k$ SimRank query. The main idea is described as follows. Given $v$, TopSim firstly finds all $v_0$ reachable from $v$ with exact $l$ steps following \emph{in-edges}, where $l$ starts from 1 and increase by 1 once all such $v_0$ are found. For each $v_0$, find all $u$ reachable from $v_0$ in exact $l$ steps following \emph{out-edges}. Moreover, $u$ must not be any node in path $v_0 \rightsquigarrow v$. Then the probability of $v_0 \rightsquigarrow v, v_0 \rightsquigarrow u$ is aggregated into $score(u,v)$, an estimation of $s(u,v)$. The algorithm stops when the gap between $k$-th and $(k+1)$-th largest score exceeds the upper bound of score any node can gain within $l$ steps, in fact, ${(\frac{c}{D})}^{l+1}$, where $c$ is the decay factor and $D$ is the average degree of the graph. They also propose several optimization algorithms to improve the speed, some with trade of accuracy.

Unfortunately, we have to point out that TopSim fails to compute an correct estimation of SimRank scores. Firstly, setting the upper bound at step $l$ to be ${(\frac{c}{D})}^{l+1}$ may result in some error, for that almost all real-world graphs have their degree distributions obeying power law. This means that there are lots of vertices have degree smaller than $D$, and the upper bound may be too optimistic to stop so early than the trivial one, i.e, $c^{l+1}$, which can make the algorithm much slower. More importantly, preventing $u$ to be any node in $v_0 \rightsquigarrow v$ can be proved neither the necessary nor the sufficient condition for computing SimRank. Details can be refered to our solution.
\subsection{Single Pair and Single Source SimRank}
Methods belong to type II should compute single pair or single source SimRank efficiently, which is the bottleneck of the top-$k$ SimRank problem, and only another top-$k$ selection is needed to get our result. The fastest two to date are the Monte Carlo method \cite{FRCS05} and SLING \cite{TX16}, with both can handle single pair and single source queries. For the Monte Carlo method, each vertex generates a fixed number of random walks, say $n_w$, stored efficiently in the \emph{fingerprint graph(FPG)}. To support single pair query, given $u, v$, the method retrieves $u$ and $v$'s random walks from \emph{FPG}, and trying to meet the $i$-th random walk of $u$ with the $i$-th of $v$'s. Note that the random walks are all truncated at step $t$ for computation efficiency. If two random walks meet at their $\tau$-th step, the SimRank score is added by $\frac{c^{\tau}}{n_w}$. Formally,
\begin{equation}
\hat{s}(u,v)=\frac{1}{n_w} \sum_{i=1}^{n_w}{c^{\tau_i}}
\end{equation}
where $\tau_i$ is number of steps the two $i$-th random walks meet($\tau_i$ is set to $\infty$ if they never meet in $t$ steps). The single source query is simply handled by doing $n-1$ single pair queries. For the top-$k$ SimRank, it's sufficient to sort and retrieve the $k$ largest score from the result of single source query.
\cite{FRCS05} gives an analysis of approximation error, while \cite{TX16} refines it by making up the missed analysis for truncation of random walks. \cite{TX16} shows to guarantee that with at least $1-\delta$ probability all pairs of $u$ and $v$ satisfy $\left\lvert \hat{s}(u, v)-s(u, v) \right\rvert \leq \varepsilon$, it needs
\begin{equation*}
t > \mathrm{log}_c \frac{\varepsilon}{2}, n_w \ge \frac{14}{3 \e^2} \left(\log \frac{2}{\delta} + 2 \log n\right)
\end{equation*}

SLING \cite{TX16} proposes a new idea for single pair and single source queries, by introducing an new interpretation of SimRank. By incorporating the decay factor $c$ into random walks, the notion of $\sqrt{c}$-walk explains random surfer as \\
(1)At each step of the surfer, stop with probability $1-\sqrt{c}$; \\
(2)Otherwise, do one step random walk.

Based on this notion they introduce three main ingredients for SimRank query. Firstly a dynamic programming algorithm is proposed to compute the sum of probabilities for all walks from $v$ to $u$ (following in-edges) with exactly $l$ steps, for each $v$ and all possible $l$. Thanks to the idea of $\sqrt{c}$-walk, they manage to prove in fact there are only $O(\frac{1}{\varepsilon})$ items ineligible for each $v$ (stored as $H(v)$), which is no smaller than $\varepsilon$. Secondly they interpret the "\emph{first meeting}" of random walks from $u$ and $v$ at $w$ (in $l$-th step) as
\begin{equation*}
h^{(\l)}(u, w) \cdot d_w \cdot h^{(\l)}(v, w)
\end{equation*}
where $d_w$ is the probability of two $\sqrt{c}$-walks starting from $w$ never meet afterwards. A sampling-based algorithm is used to estimate $d_w$ for each $w \in V$. At last these two techniques are combined to give the estimation of SimRank:
\begin{equation*}
\hat{s}(u, v) = \sum_{\l = 0}^\infty \sum_{w = 1}^n \left(h^{(\l)}(u, w) \cdot d_w \cdot h^{(\l)}(v, w)\right).
\end{equation*}

A few theorems prove the algorithm can guarantee $\varepsilon$ absolute error for all $\hat{s}(u, v)$ with at least $1-\delta$ probability, with only $O(\frac{1}{\varepsilon})$ time for single pair query and $O(\frac{n}{\varepsilon})$ (or $O(m{\mathrm{log}}^2\frac{1}{\varepsilon})$ but performs better in practice) for single source query, both being asymptotic optimal.
However, both two methods have several shortcomings for top-$k$ queries. They both need preprocessing, for that Monte Carlo method has to generate and store random walks for each vertex, and SLING needs to compute $H(v)$ and $d_v$ for each $v \in V$. Moreover, it needs $O(\frac{n}{\varepsilon})$ storage to keep these information for SLING, which is too large for typical $\varepsilon$, for example, $0.01$. Another problem of these methods is they are not tailored for the top-$k$ queries, it's unnecessary to compute the similarity of all vertices with respect to a given $v$, as mentioned in \cite{LeeLY12}, since most vertices have very low similarity scores while computing them cost a lot of time.
\subsection{All-Pair SimRank}
All the methods for all-pair SimRank can be naively applied to top-$k$ queries given source node $v$, by simply retrieve the line corresponding to $v$ and do a top-$k$ selection. It's obvious that all methods of this kind are much slower than any type I or II method, since they need to compute $n^2$ items, which will cost $\Omega(\frac{n^2}{\varepsilon})$ to achieve $\varepsilon$ error. Methods fall into this type includes the Power Method \cite{JW02} introduced with SimRank, as well as some optimizations such as \cite{LVGT10} and \cite{YZL12}.

For other related works, refer to Section ?. They solve basically different problems to single pair, single source or top-$k$ queries, and some of them fail to compute the correct SimRank score or achieve no theoretical guarantee on the results. 
